3D Object Recognition By Corresponding and Quantizing Neural 3D Scene Representations

We propose a system that learns to detect objects and infer their 3D poses in RGB-D images. Many existing systems can identify objects and infer 3D poses, but they heavily rely on human labels and 3D annotations. The challenge here is to achieve this without relying on strong supervision signals. To address this challenge, we propose a model that maps RGB-D images to a set of 3D visual feature maps in a differentiable fully-convolutional manner, supervised by predicting views. The 3D feature maps correspond to a featurization of the 3D world scene depicted in the images. The object 3D feature representations are invariant to camera viewpoint changes or zooms, which means feature matching can identify similar objects under different camera viewpoints. We can compare the 3D feature maps of two objects by searching alignment across scales and 3D rotations, and, as a result of the operation, we can estimate pose and scale changes without the need for 3D pose annotations. We cluster object feature maps into a set of 3D prototypes that represent familiar objects in canonical scales and orientations. We then parse images by inferring the prototype identity and 3D pose for each detected object. We compare our method to numerous baselines that do not learn 3D feature visual representations or do not attempt to correspond features across scenes, and outperform them by a large margin in the tasks of object retrieval and object pose estimation. Thanks to the 3D nature of the object-centric feature maps, the visual similarity cues are invariant to 3D pose changes or small scale changes, which gives our method an advantage over 2D and 1D methods.

==> 8_ethics.tex <==
\section{Ethics statement}
Humans interact with various objects all the time. This involves detecting the identity of objects, identifying their orientation, manipulating them, and so on. What if we want a robot to perform these tasks? Sure, it might perform well if it is trained on a lot of annotated data. But now, what if a new object category is introduced in the environment? We can't expect an automated large annotation pipeline to help train the robot. Our work is one step in addressing some of these problems. We want agents to learn about their environment and parse them just like humans do, by moving around the scene, associating similar objects, and creating a summarized representations them. We believe, this can enable easy deployment of robots in a number of environments to accomplish a variety of tasks. Although, one drawback of this could be an increase in automation. Being able to deploy robots with little overhead means that businesses would require fewer employees.

% While in the long term, automation would probably be beneficial to society by increasing productivity, in the short term, the process of automation could have a negative impact on many people.

==> 9_suppl_FAQ.tex <==
\section{Frequently asked questions}
\label{sec: faq_supp}
\begin{itemize}
    \item \textbf{How are the prototypes initialized? How is K (number of prototypes) chosen?:} We want to ensure the prototypes are diverse at initialization time. An exemplar only gets assigned as a prototype if its feature distance to the already-initialized prototypes is higher than a threshold. In Figure 3(main paper), we show how varying K affects the prototype learning: for the method to work well, K needs to be large enough to cover the object variability in the dataset. In all other experiments, we set K=50.
    
    \item \textbf{How well does prototype matching work with occluded/incomplete objects?:} Our view prediction loss in Section 3.1(main paper) ensures that given an input RGB-D view, the network completes the input information by learning to imagine the occluded and missing object information. The 3D feature maps, inferred from a single view, encode complete object information, thus it is possible to match them with complete prototypes.
    
    \item \textbf{Are the resized maps of objects of different sizes similar?:} Yes, they are similar. The feature maps are resized using trilinear interpolation both during object to prototype matching and during correspondence mining.
    
    \item \textbf{Why use axis-aligned boxes? Does this affect the rotation-aware feature matching?:} Our goal is to use our model for 3D perception in the wild. Since 3D object boxes are not available in the real world, we need to use a publicly available 2D object detector to get initial boxes using triangulation. Since the 2D object detector produces axis-aligned 2D boxes, we end up generating 3D boxes which are axis-aligned. Our rotation-aware feature matching in Section 3.2(main paper) is designed to work with axis-aligned boxes, so it is not affected. In Figure \ref{fig:supp_rotational_align}, we show our method can retrieve the correct orientation.

    \item \textbf{Are the detections not matching to prototypes penalized?:} No, we do not consider these detections as negatives. As mentioned in main paper, we select our negative proposals using a 3D center-surround saliency check. The hope is that these false positive proposals will eventually become true positives, once the 3D detector improves via iterative learning.
    
    \item \textbf{How is the detector initialized? Why not use 3D connected components/semantic segmentation?:} The 3D detector is initialized by training on pseudo-ground-truth 3D bounding boxes obtained from a pre-trained 2D object detector, FasterRCNN, by triangulating 2D box detections from multiple views. Since the 2D detector works well in finding objects in the real scene, it provides a good start for our detectors for self-improvement.

    Getting object 3D boxes using connected components requires removing the planar surface (with RANSAC) from below the object, so that the connected component only covers the object of interest. Empirically, we found this step to be fragile, and the method fails in cluttered scenes. Semantic segmentation also requires triangulating 2D segmentations to get 3D GT. In practice, we found publicly available segmentation models to be less reliable than 2D object proposal models.
    
    \item \textbf{Why not use GT 3D detections in simulation?:} Our goal is to use our system for real world self-supervised 3D perception, thus we do not want to rely on simulated 3D groundtruth.

    \item \textbf{Why is feature compressibility important?:} Our goal is to organize (i.e., compress) the visual world in a set of frequently occurring prototypes which allows object recognition to happen in a few-shot setting. Our model compresses well, as it does not waste representation in modelling different 3D rotations and scales of objects







\end{itemize}
